SuperMann: a superlinearly convergent algorithm for finding fixed points of nonexpansive operators

Operator splitting techniques have recently gained popularity in convex optimization problems arising in various control fields. Being fixed-point iterations of nonexpansive operators, such methods suffer many well known downsides, which include high sensitivity to ill conditioning and parameter selection, and consequent low accuracy and robustness. As universal solution we propose SuperMann, a Newton-type algorithm for finding fixed points of nonexpansive operators. It generalizes the classical Krasnosel'skii-Mann scheme, enjoys its favorable global convergence properties and requires exactly the same oracle. It is based on a novel separating hyperplane projection tailored for nonexpansive mappings which makes it possible to include steps along any direction. In particular, when the directions satisfy a Dennis-Mor\'e condition we show that SuperMann converges superlinearly under mild assumptions, which, surprisingly, do not entail nonsingularity of the Jacobian at the solution but merely metric subregularity. As a result, SuperMann enhances and robustifies all operator splitting schemes for structured convex optimization, overcoming their well known sensitivity to ill conditioning.

==> TeX/Alg/Broyden_NestedLoops.tex <==
\begin{algorithmic}
	\STATE{\(d\gets H_k^0d_k\)}%
	\FOR{\(i=1\ldots m\)}%
		\STATE{%
			\(y_i'\gets H_k^0 y_i\)\,;\quad
			\textbf{for } \(j=1\ldots i-1\) \textbf{ do } 
			\(
				y_i'
			{}\gets{}
				y_i'
				{}+{}
				\frac{
					\innprod{y_i'}{s_j}
				}{
					\innprod{y_j'}{s_j}
				}
				\bigl(s_j-y_j'\bigr)
			\)
			\textbf{ end for}%
		}%
		\STATE{%
			Select \(\vartheta_k^i\in[0,2]\) based on
			\(
				\gamma_k^i
			{}={}
				\frac{\innprod{y_i'}{s_i}}{\|s_i\|^2}
			\)%
		}%
		\STATE{%
			\(
				y_i'
			{}\gets{}
				(1-\vartheta_k^i)s_i + \vartheta_k^iy_i'
			\)\,;\quad
			\(
				d
			{}\gets{}
				d
				{}+{}
				\frac{
					\innprod{d}{s_i}
				}{
					\innprod{y_i'}{s_i}
				}
				\bigl(s_i-y_i'\bigr)
			\)%
		}%
	\ENDFOR{}%
\end{algorithmic}%


==> TeX/Alg/LBroyden.tex <==
\begin{algorithmic}[1]
	\Require{%
		\(m,k\in\N_{\geq1}\),~
		\(d_k\in\HH\),~
		\(H_k^0\in\linop\),~
		\((s_{k-1},y_{k-1})\),%
	}%
	\item[]{%
		\hspace*{0pt}\textfillwidthof{\textbf{Initialize:}}{}
		buffers \({\bf s},{\bf y}\) with \(\dim({\bf s})=\dim({\bf y})\leq\min\set{m,k-1}\)%
	}%
	\Provide{%
		\(d=H_kd_k\),~
		new buffers \({\bf s},{\bf y}\)%
	}%
	\STATE{%
		\textbf{if } \(\dim({\bf s})<m\)
		\textbf{ then } \({\bf s}\gets[{\bf s},s_{k-1}]\),~ \({\bf y}\gets[{\bf y},y_{k-1}]\)%
	}%
	\STATE{%
		\textbf{else } \({\bf s}\gets[{\bf s}_2\ldots {\bf s}_m,s_{k-1}]\),~ \({\bf y}\gets[{\bf y}_2\ldots {\bf y}_m,y_{k-1}]\) \textbf{ end if}%
	}%
	\STATE{\(d\gets H_k^0d_k\)}%
	\FOR{\(i=1\ldots \dim({\bf s})\)}%
		\STATE{\(y_i'\gets H_k^0 y_i\)}%
		\FOR{\(j=1\ldots i-1\)}%
			\STATE{\(
				y_i'
			{}\gets{}
				y_i'
				{}+{}
				\frac{
					\innprod{y_i'}{{\bf s}_j}
				}{
					c_j
				}
				\bigl({\bf s}_j-y_j'\bigr)
			\)}%
		\ENDFOR{}%
		\COMMENT{up to here, \(y_i'=H_k^iy_{k-m+i}\)}%
		\STATE{\(
			c_i
		{}\gets{}
			\innprod{y_i'}{{\bf s}_i}
		,~~~
			\nu_i
		{}\gets{}
			\|{\bf s}_i\|^2
		,~~~
			\gamma_k^i
		{}\gets{}
			\nicefrac{c_i}{\nu_i}
		\)}%
		\STATE{%
			Select \(\vartheta_k^i\in[0,2]\) based on \(H_k^i\), \(({\bf s}_i,{\bf y}_i)\) and \(\gamma_k^i\)%
		}%
		\STATE{\(y_i'\gets(1-\vartheta_k^i){\bf s}_i + \vartheta_k^iy_i'\)}%
		\COMMENT{now, \(y_i'=H_k^i\bigl((1-\vartheta_k^i)B_k^is_{k-m+i}+\vartheta_k^iy_{k-m+i}\bigr)\)}%
		\STATE{\(
			\fillwidthof[l]{y_i'}{c_i}
		{}\gets{}
			(1-\vartheta_k^i)\nu_i + \vartheta_k^ic_i
		\)}%
		\STATE{\(
			\fillwidthof[l]{y_i'}{d}
		{}\gets{}
			d
			{}+{}
			\frac{
				\innprod{d}{{\bf s}_i}
			}{
				c_i
			}
			\bigl({\bf s}_i-y_i'\bigr)
		\)}%
	\ENDFOR{}%
\end{algorithmic}


==> TeX/Alg/RBroyden_unscaled.tex <==
\begin{algorithmic}[1]
	\Require{%
		\(m,k\in\N_{\geq1}\),~
		\(d_k\in\HH\),~
		\(H_k^0\in\linop\),~
		\((s_{k-1},y_{k-1})\)%
	}%
	\item[]{%
		\hspace*{0pt}\textfillwidthof{\textbf{Initialize:}}{}
		buffers \(S,\tilde S,C\) with same dimension \(\leq\min\set{m,k-1}\)%
	}%
	\Provide{%
		\(d=H_kd_k\),~
		\(H_{k+1}^0\),~
		new buffers \(S,\tilde S,C\)%
	}%
	\vspace*{3pt}%
	\STATE{%
		\textbf{if } \(\dim(C)=m\)
		\textbf{ then }
		\(
			S,\tilde S,C\gets[\,]
		\,;\quad
		\)%
		select \(H_k^0\in\linop\)
		\textbf{ end if}%
	}%
	\STATE{\(
		d\gets H_k^0d_k
	\,;\quad
		\tilde s\gets H_k^0y_{k-1}
	\)}%
	\FOR{\(i=1\ldots \dim(S)\)}%
		\STATE{\(
			\tilde s
		{}\gets{}
			\tilde s
			{}+{}
			\frac{
				\innprod{\tilde s}{S_i}
			}{
				C_i
			}
			\tilde S_i
		\,;\quad
			d
		{}\gets{}
			d
			{}+{}
			\frac{
				\innprod{d}{S_i}
			}{
				C_i
			}
			\tilde S_i
		\)}%
	\ENDFOR{}%
	\STATE{%
		\(\fillwidthof[l]{S}{\nu}\gets\|s_{k-1}\|^2\)%
		\,;\quad
		\(c\gets\innprod{\tilde s}{s_{k-1}}\)%
		\,;\quad
		select \(\vartheta_{k-1}\in[0,2]\) based on
		\(
			\gamma_{k-1}
		{}={}
			\nicefrac c\nu
		\)%
	}%
	\STATE{\(
		\fillwidthof[l]{S}{c}\gets(1-\theta_{k-1})\nu+\theta_{k-1}c
	\,;\quad
		\tilde s\gets\vartheta_{k-1}(s_{k-1}-\tilde s)
	\,;\quad
		d\gets d + \frac{\innprod{d}{s_{k-1}}}{c}\tilde s
	\)}%
	\STATE{\(
		\fillwidthof[l]{S}{S}\gets [S,s_{k-1}]
	\,;\quad
		\tilde S\gets [\tilde S,\tilde s]
	\,;\quad
		C\gets [C,c]
	\,;\quad
		H_{k+1}^0\gets H_k^0
	\)}%
\end{algorithmic}


==> TeX/Alg/RBroyden_wordy.tex <==
\begin{algorithmic}[1]
	\STATE\label{alg:RBroyden_wordy:init}
		initialize \(d_k\gets-Rx_k\) and \(\tilde s_{k-1}\gets y_{k-1}\)
	\STATE
		iterate sequentially over the buffer (\(i=k-m'\ldots k-2\))
		\ifieee
			\[
				\begin{array}{l@{{}\gets{}}rl}
					\tilde s_{k-1}
				&
					\tilde s_{k-1}
				&
					{}+{}
					\frac{
						\innprod{s_i}{\tilde s_{k-1}}
					}{
						\innprod{s_i}{\tilde s_i}
					}
					(s_i-\tilde s_i)
				\\
					d_k
				&
					d_k
				&
					{}+{}
					\frac{
						\innprod{s_i}{d_k}
					}{
						\innprod{s_i}{\tilde s_i}
					}
					(s_i-\tilde s_i)
				\end{array}
			\]
		\else
			\[
				\tilde s_{k-1}
			{}\gets{}
				\tilde s_{k-1}
				{}+{}
				\frac{
					\innprod{s_i}{\tilde s_{k-1}}
				}{
					\innprod{s_i}{\tilde s_i}
				}
				(s_i-\tilde s_i)
			\quad\text{and}\quad
				d_k
			{}\gets{}
				d_k
				{}+{}
				\frac{
					\innprod{s_i}{d_k}
				}{
					\innprod{s_i}{\tilde s_i}
				}
				(s_i-\tilde s_i)
			\]
		\fi
	\STATE
		compute \(\vartheta_{k-1}\) as in \eqref{eq:PowellTheta} and finalize
		\ifieee
			\[
				\begin{array}{l@{{}\gets{}}l}
					\tilde s_{k-1}
				&
					(1-\vartheta_{k-1})s_{k-1}
					{}+{}
					\vartheta_{k-1}\tilde s_{k-1}
				\\
					d_k
				&
					d_k
					{}+{}
					\frac{
						\innprod{s_{k-1}}{d_k}
					}{
						\innprod{s_{k-1}}{\tilde s_{k-1}}
					}
					(s_{k-1}-\tilde s_{k-1})
				\end{array}
			\]
		\else
			\[
				\tilde s_{k-1}
			{}\gets{}
				(1-\vartheta_{k-1})s_{k-1}
				{}+{}
				\vartheta_{k-1}\tilde s_{k-1}
			\quad\text{and}\quad
				d_k
			{}\gets{}
				d_k
				{}+{}
				\frac{
					\innprod{s_{k-1}}{d_k}
				}{
					\innprod{s_{k-1}}{\tilde s_{k-1}}
				}
				(s_{k-1}-\tilde s_{k-1})
			\]
		\fi
	\STATE
		empty the buffer \((s_i,\tilde s_i)\) if full (\ie if \(m'=m\)), or append \((s_{k-1},\tilde s_{k-1})\) otherwise.
\end{algorithmic}



==> TeX/Alg/RGKM.tex <==
\begin{algorithmic}[1]%
\newcommand\keyfont[1]{\textsc{#1}}%
\item[]%
	\begin{tabularx}{\linewidth}{@{}l@{~~}X@{}}
			\keyfont{Require}%
		&
			\(x^0\in\HH\),~
			\(\beta,\sigma\in(0,1)\).%
		\\
			\keyfont{Initialize}%
		&
			\(k=0\),~
			\(I=\set{1\ldots N}\).%
	\end{tabularx}
\STATE\label{step:RGKM:initial}%
	\keyfont{If } \(I=\emptyset\), \keyfont{ then stop}%
\STATE%
	Sample a random index \(j\in I\)%
\STATE%
	\keyfont{If } \(R_jx^k=0\), \keyfont{ then ~set } \(I\gets I\setminus\set j\) and go to step \ref{step:RGKM:initial}%
\STATE%
	Set \(I\gets\set{1\ldots N}\) and select an update direction \(d_j\in\HH_j\)%
\STATE\label{step:RGKM:LS}%
	Let \(\tau=\beta^m\), with \(m\in\N\) the smallest such that \(w=x^k+\tau\imm d_j\) satisfies
	\[
		\rho_j
	{}\coloneqq{}
		\innprod{R_jw}{x_j^k-T_jw}_{\HH_j}
	{}\geq{}
		\sigma\|R_jw\|_{\HH_j}\|R_jx^k\|_{\HH_j}
	\]
\STATE%
	Let \(x^{k+1}\in\HH\) be defined as
	\[	
		x^{k+1}_i
	{}\coloneqq{}
		\begin{cases}[c@{~~\text{if }}l]
			x^k_i & i\neq j\\
			x^k_j - \frac{\rho_j}{\|R_jw\|\mathrlap{_{\HH_j}}}~~R_jw & i=j.
		\end{cases}
	\]
\STATE%
	Set \(k\gets k+1\) and go to step \ref{step:RGKM:initial}.
\end{algorithmic}


==> TeX/Alg/SS.tex <==
\begin{algorithmic}[1]
	\STATE{%
		Select a pos.def. matrix \(B_k\) and let \(d_k=-B_k^{-1}Rx_k\)
	}\label{step:SS:initial}%
	\STATE{%
		\(w_k=x_k+\tau_kd_k\) with \(\tau_k\in(0,1]\) s.t.
		\(
			-\innprod{Rw_k}{d_k}
		{}\geq{}
			\sigma_k\|d_k\|^2
		\),
		\ie
		\begin{equation}\label{eq:SS-LS}
			\|Rw_k\|^2
			{}-{}
			\innprod{Rw_k}{x_k-Tw_k}
		{}\leq{}
			-\sigma_k\tau_k
			\|d_k\|^2
		\end{equation}
	}%
	\STATE{%
		\(x_{k+1}=\proj_{H_k}x_k\) where
		\begin{align}
		\label{eq:SS-Hk}
			H_k
		{}\coloneqq{} &
			\set{z\in\HH}[
				\innprod{Rw_k}{z-w_k}
			{}\leq{}
				0
			]
		\\
		\nonumber
		{}={} &
			\set{z\in\HH}[
				\|Rw_k\|^2
				{}-{}
				\innprod{Rw_k}{z-Tw_k}
			{}\geq{}
				0
			]
		\end{align}
	}%
	\STATE{%
		\(k\gets k+1\), and go to \cref{step:SS:initial}%
	}%
\end{algorithmic}



==> TeX/Alg/Temp.tex <==
	\Require{%
		\(m,k\in\N_{\geq1}\),~
		\(d_k\in\HH\),~
		\(H_k^0\in\linop\),~
		\((s_{k-1},y_{k-1})\)%
	}%
	\item[]{%
		\hspace*{0pt}\textfillwidthof{\textbf{Initialize:}}{}
		buffers \(S,\tilde S,C\) with same dimension \(\leq\min\set{m,k-1}\)%
	}%
	\Provide{%
		\(d=H_kd_k\),~
		\(H_{k+1}^0\),~
		new buffers \(S,\tilde S,C\)%
	}%
	\vspace*{3pt}%
	\STATE{%
		\textbf{if } \(\dim(C)=m\)
		\textbf{ then }
		\(
			S,\tilde S,C\gets[\,]
		\,;\quad
		\)%
		select \(H_k^0\in\linop\)
		\textbf{ end if}%
	}%
	\STATE{\(
		d\gets H_k^0d_k
	\,;\quad
		\tilde s\gets H_k^0y_{k-1}
	\)}%
	\FOR{\(i=1\ldots \dim(S)\)}%
		\STATE{\(
			\tilde s
		{}\gets{}
			\tilde s
			{}+{}
			\frac{
				{\innprod{\tilde s}{S_i}\!}_2
			}{
				C_i
			}
			\tilde S_i
		\,;\quad
			d
		{}\gets{}
			d
			{}+{}
			\frac{
				{\innprod{d}{S_i}\!}_2
			}{
				C_i
			}
			\tilde S_i
		\)}%
	\ENDFOR{}%
	\STATE{%
		\(\fillwidthof[l]{S}{u}\gets Ps_{k-1}\)%
		\,;\quad
		\(\nu\gets{\innprod{s_{k-1}}{u}\!}_2\)%
		\,;\quad
		\(c\gets{\innprod{\tilde s}{u}\!}_2\)%
		\,;\quad
		select \(\vartheta_{k-1}\in[0,2]\) based on
		\(
			\gamma_{k-1}
		{}={}
			\nicefrac c\nu
		\)%
	}%
	\STATE{\(
		\fillwidthof[l]{S}{c}\gets(1-\theta_{k-1})\nu+\theta_{k-1}c
	\,;\quad
		\tilde s\gets\vartheta_{k-1}(s_{k-1}-\tilde s)
	\,;\quad
		d\gets d + \frac{{\innprod{d}{u}\!}_2}{c}\tilde s
	\)}%
	\STATE{\(
		\fillwidthof[l]{S}{S}\gets [S,u]
	\,;\quad
		\tilde S\gets [\tilde S,\tilde s]
	\,;\quad
		C\gets [C,c]
	\,;\quad
		H_{k+1}^0\gets H_k^0
	\)}%



==> TeX/Alg/thetaChoice.tex <==
\begin{algorithmic}[]
	\IF{\(\gamma_k\geq1\)}%
		\STATE{%
			~~\textbf{if }
			\(\alpha|\delta_k|\leq\innprod{y_k}{s_k}\)
			\textbf{ then }
			\(\theta_k=1\)%
		}%
		\STATE{%
			~~\textbf{else }
			\(\theta_k=\delta_k\frac{1-\sigma_k\alpha}{\delta_k-\innprod{y_k}{s_k}}\)
			~~\textbf{end if}%
		}%
	\ELSE{}%
		\STATE{%
			~~\textbf{if }
			\((1+\alpha)\delta_k\geq2\innprod{y_k}{s_k}\)
			\textbf{ then }~
			\(\theta_k=\frac{1-\bar\theta}{1-\gamma_k}\)%
		}%
		\STATE{%
			~~\textbf{else }
			\(
				\theta_k
			{}={}
				\sigma_k\min\set{
					\sigma_k\frac{1-\sigma_k\bar\theta}{1-\gamma_k},~
					|\delta_k|\frac{1-\sigma_k\alpha}{\delta_k-\innprod{y_k}{s_k}}
				}
			\)
			~~\textbf{end if}%
		}%
	\ENDIF{}\textbf.\hfill\qed%
\end{algorithmic}


==> TeX/Tables/LargeScaleSpringMass.tex <==
\footnotesize
\newcommand\x{\bf\(\times\)}%
\setlength\tabcolsep{1.5pt}%
\begin{tabular}[t]{@{}r@{\,\,}}
	\vphantom{\(\trans L\)}\\
	\vphantom{\(K32\) \(N75\)}\\
	\vspace*{1pt}\vphantom{avg}\\
	SuperVC\\
	VC\\
	Mosek
\end{tabular}%
\begin{tabular}[t]{@{}|rrr|@{}}
	\multicolumn{3}{c}{time (s)}\\%
\hline
		\multicolumn{3}{|c|}{\(K32\) \(N75\)}%
\\
		min & avg & max
\\
\hline
	\rowcolor{gray!20}\vphantom{\(X^X\)}%
	\bf3.0 &\bf3.9 &\bf4.9\\
	\rowcolor{gray!10}%
	4.2 & 5.1 & 8.6\\
	59.8 & 85.2 & 104.2\\
\hline
\end{tabular}%
~%
\begin{tabular}[t]{@{}| rrr | rrr | rrr |@{}}
	\multicolumn{9}{c}{\# of calls to \(L\) and \(\trans L\) (\(\cdot10^3\))}\\%
\hline
	\multicolumn{3}{|c|}{\(K32\) \(N100\)}&%
	\multicolumn{3}{c|}{\(K64\) \(N75\)}&%
	\multicolumn{3}{c|}{\(K64\) \(N100\)}%
\\
		  min & avg & max
		& min & avg & max
		& min & avg & max
\\
\hline
	\rowcolor{gray!20}\vphantom{\(X^X\)}%
	11.5 & 16.9 & 24.7	& 20.0 & 22.9 & 30.9	& 12.7 & 19.5 & 26.1 \\
	\rowcolor{gray!10}%
	31.2 & 38.3 & 43.9	& 34.4 & 39.3 & 49.3	& 29.9 & 33.8 & 36.7 \\
\hline
	\multicolumn{9}{c}{}%
\end{tabular}%


==> TeX/Text/Broyden/Broyden.tex <==
%\begin{thm}[{\cite[Thm. 3.2]{more1976global}}]
%Suppose that \hl{$\func{F}{\R^n}{\R^n}$ is linear and Lipschitz continuously differentiable in a neighborhood} of \(x_\star\in\zer F\) and that \(G_\star\coloneqq\jac F{x_\star}\) is \hl{strongly nonsingular}.
%Then, for any \(x_0\in\HH\) close enough to \(x_\star\) and \(B_0\in\linop\) close enough to \(G_\star\) such that \(B_0-G_\star\) is a Hilbert-Schmidt operator, the modified Broyden method produces a sequence of iterates \(\seq{x_k}\) that converges to \(x_\star\) at \(Q\)-superlinear rate.
%\end{thm}
%\begin{thm}[{\cite[Thm. 3.5]{sachs1986broyden}}]
%Suppose that \(\func F\HH\HH\) is \hl{Lipschitz continuously differentiable in a neighborhood} of \(x_\star\in\zer F\) and that \(G_\star\coloneqq\jac F{x_\star}\) is \hl{strongly nonsingular}.
%Then, for any \(x_0\in\HH\) close enough to \(x_\star\) and \(B_0\in\linop\) close enough to \(G_\star\) such that \(B_0-G_\star\) is a Hilbert-Schmidt operator, the \hl{(non-modified)} Broyden method is well defined and produces a sequence of iterates \(\seq{x_k}\) that converges to \(x_\star\) at \(Q\)-superlinear rate.
%\end{thm}
For simplicity, in this section we will consider only finite dimensional Hilbert spaces \(\HH\).
For efficiently solving a nonlinear equation
\begin{equation}\label{eq:NonlinEq}
	\text{given}~~
	\func F\HH\HH
	\qquad\text{find}~~
	x_\star\in\zer F,
\end{equation}
starting from an invertible operator \(B_0\in\linop\) quasi-Newton methods operate low-rank updates satisfying the \emph{secant condition}
\begin{equation}\label{eq:Secant}
	B_{k+1}s_k
{}={}
	y_k
\quad\text{with}\quad
	\begin{cases}
		s_k & {}= x_{k+1}- x_k \\
		y_k & {}= F(x_{k+1}) - F(x_k)
	\end{cases}
\end{equation}
and prescribe recursive iterations of the form
\begin{equation}\label{eq:xQN}
	x_{k+1}
{}={}
	x_k-B_k^{-1}F(x_k).
\end{equation}
Under some regularity condition of \(F\) at the solution, quasi-Newton schemes are locally superlinearly convergent yet, differently from Newton methods, without requiring the computation of first-order information.
There are many quasi-Newton updates available, the BFGS formula being the most popular, but many of them are provably well performing only under the assumption of symmetricity (and nonsingularity) of the Jacobian at the solution.
Symmetricity is ensured, for instance, when the objective is the minimization of a convex smooth function \(f\); the problem is indeed equivalent to solving the nonlinear equation \(\nabla f(x)=0\), whose Jacobian is a symmetric matrix provided \(f\in C^2\).

Unfortunately this is often not the case, as it happens for meaningful applications of problem \eqref{eq:Problem}.
Broyden's method offers a universal alternative that does not necessitate symmetricity; the standard Broyden's update is of the form
\begin{align}
\label{eq:StandardBroyden}
	B_{k+1}
{}={} &
	B_k
	{}+{}
	\frac{
		(y_k-B_k s_k)
	}{
		\|s_k\|^2
	}
	\otimes s_k
\intertext{%
	and if \(B_k\in\linop\) is nonsingular, then so is \(B_{k+1}\) as long as \(\innprod{B_k^{-1}y_k}{s_k}\neq 0\).
	Indeed, letting \(H_k\coloneqq B_k^{-1}\), from the Sherman-Morrison-Woodbury identity we obtain the \emph{inverse} Broyden's update formula%
}
\label{eq:BroydenInverse}
	H_{k+1}
{}={} &
	H_k
	{}+{}
	\frac{
		s_k
		{}-{}
		H_ky_k
	}{
		\innprod{H_ky_k}{s_k}
	}
	\otimes
	\bigl(
		\trans{H_k}
		s_k
	\bigr).
\end{align}
\(B_{k+1}\) is simply the operator \emph{closest} to \(B_k\) with respect to the Hilbert-Schmidt metric \(\|{}\cdot{}\|_{\HS[]}\) that satisfies \eqref{eq:Secant}, namely,
\begin{align}
\label{eq:StandardBroydenProjection}
	B_{k+1}
{}={}
	\proj_{S_k}
	(B_k)
{}\coloneqq{} &
	\argmin_{B\in S_k}\tfrac 12\|B-B_k\|_{\HS[]}^2, 
\shortintertext{where}
	S_k
{}\coloneqq{} &
	\set{B\in\linop}[Bs_k=y_k]
\end{align}
is the space of bounded operators satisfying the secant condition \eqref{eq:Secant}.
If \(\HH\) is infinite dimensional, then \(\HS\subsetneqq\linop\) and the projection in \eqref{eq:StandardBroydenProjection} is to be interpreted as \(B_k+S\) where \(S\in\HS\) is the closest to zero in \(\HS\) such that \(B_k+S\in S_k\).
\cite{artacho2014local} describes this in detail with more formalism and explains how properties of the projection can be extended in this case.
However, for the sake of simplicity we limit the work to finite dimensional Hilbert spaces, where we may simply consider the space \(\HS\) as \(\linop\) endowed with a different, yet equivalent, metric.

The standard least conservative assumptions to ensure local superlinear convergence of Broyden iterations \eqref{eq:xQN} require that
\begin{enumerate}[%
	label={A. \arabic*)},
	ref={Assumption \arabic*)},
]
	\item\label{item:invertible}
		all Broyden operators \(B_k\) are invertible;
	\item\label{item:convergence}
		the sequence \(\seq{x_k}\) converges to a solution \(x_\star\in\zer F\);
	\item\label{item:calm}
		the semiderivative \(\Bjac F{}\) is locally Lipschitz continuous at \(x_\star\) (and in particular \(F\) is strictly differentiabile at \(x_\star\));
	\item\label{item:nonsing}
		the Jacobian \(\jac F{x_\star}\) is nonsingular.
\end{enumerate}
Our ultimate goal is to implement Broyden-like directions in the \refSM[] when \(\id-F\) is a nonexpansive operator.
In this setting many simplifications can be made; we briefly outline them here, deferring more details to \Cref{thm:SuperMannBroyden}.

\Cref{item:invertible} is easily addressable thanks to the work pioneered in \cite{powell1970numerical} for the solution of linear systems and later generalized in \cite{more1976global} also for locally smooth equations, which furnishes a suitable modification of Broyden's update \eqref{eq:StandardBroyden} that ensures the sought invertibility; we will discuss this in \Cref{sec:Relaxation}.

\Cref{item:convergence} is automatically ensured by the \refSM[] as long as \(\HH\) is finite dimensional and the sequence \(\seq{B_k^{-1}}\) is bounded (cf. \cref{thm:SuperMann:xWeak}).

\Cref{item:nonsing} is typically needed to show that \(\seq{x_k}\) converges (at least) linearly, hence to infer that \(\seq{\|x_k-x_\star\|}\) is summable and finally to conclude that the Dennis-Moré condition for superlinear convergence is satisfied.
\cite{artacho2014local} generalizes this property invoking the concepts of (strong) metric (sub)regularity of \(F\) at \(x_\star\) (see also \cite{dontchev2004regularity,dontchev2009implicit} for an extensive review on these properties).
However, if \(F\) is strictly differentiable at \(x_\star\), then strong subregularity, regularity and strong regularity are equivalent to injectivity, surjectivity and invertibility of \(\jac F{x_\star}\), respectively, these conditions being all equivalent for mappings \(\func F\HH\HH\) with \(\HH\) finite dimensional.
It seems then that a certificate of superlinear convergence requires at least the limit point \(x_\star\) to be isolated in \(\zer F\), a property that rules out many interesting applications (cf. \cref{sec:SCS}).
On the other hand, in \Cref{{thm:General:Linear},{thm:SuperMann:Linear}} we provided conditions for the general framework of \Cref{alg:General}, and consequently of the \refSM[], to exhibit linear convergence rates only by requiring metric \emph{sub}regularity, a weak property that, for instance, is satisfied by any affine mapping \cite[p. 187]{dontchev2009implicit}, whereas for the other three stronger properties to hold invertibility would be necessary.
This is possible thanks to the particular structure of problem \eqref{eq:Problem}, where \(F=R\) is the residual of a nonexpansive operator, and to the ad-hoc clever interleaving of GKM and \emph{blind/educated} updates that ensure quasi-Fejér monotonicity of the generated sequence.
This kind of property is the key that allows to relax nonsingularity of \(\jac F{x_\star}\) to mere metric subregularity.

To recap, in \Cref{thm:SuperMannBroyden} we will see that when Broyden directions are used in the \refSM[], for superlinear convergence to hold the four requirements can be reduced to
\begin{enumerate}[%
	label={A. \(\arabic*'\))},
	ref={Assumption \arabic*')},
]
	\setcounter{enumi}{1}
	\item
		the sequence of Broyden operators \(\seq{B_k^{-1}}\) is bounded;
	\item
		\Cref{item:calm} holds;
	\item
		the residual \(R\) is metrically subregular at \(x_\star\).
\end{enumerate}

%\cite{sachs1986broyden} extended the result to infinite dimensional systems of locally smooth equations, but requiring the first Broyden's estimate \(B_0\) to be \emph{sufficiently close} to the Jacobian at the solution \(G_\star\).
%More precisely, \(B_0-G_\star\) needs be a Hilbert-Schmidt operator or, in other words, of finite Frobenius norm (a property that trivially holds in finite dimension).
%In this section we show that the modified scheme still enjoys the same properties for infinite dimensional systems of locally semidifferentiable equations without any assumption on \(B_0\) other than invertibility.
%Our proofs are based on the geometrical interpretation \eqref{eq:StandardBroydenProjection} and on the (firm) nonexpansiveness of the projection operator.
We first consider the general framework \eqref{eq:NonlinEq} and then tailor the results for the employment of the modified Broyden's scheme in the \refSM[].





==> TeX/Text/Broyden/LimitedMemory.tex <==
When the problem size is too large even simple linear algebra becomes computationally challenging, not to mention the memory requirements for storing big opesrators.
To overcome the issue, \emph{limited-memory} or \emph{restarted} variants of quasi-Newton schemes exist that use only the last \(m\) couples \((s_k,y_k)\), where \(m\) is a small integer typically between \(3\) and \(20\).
Memory usage is then significantly reduced, and matrix-vector products are replaced by scalar multiplications.
From a theoretical point of view these variants cannot be shown to achieve the superlinear convergence rates enjoyed by their full-memory counterparts (cf. \cref{sec:superlinear}).
However, in practice they perform extremely well, oftentimes even beating full-memory methods, and as such are ubiquitous in unconstrained smooth optimization methods.


==> TeX/Text/Broyden/LimitedMemory/LimitedMemory.tex <==
In \cite{byrd1994representations} an efficient formula tailored for Broyden's method is provided (the extension to Hilbert spaces is straightforward); we restate it here for the reader's convenience.
\begin{thm}[{\cite[Thm. 6.2]{byrd1994representations}}]
Let \(H\in\linop\) be a nonsingular starting operator, and let \(H_k\) be obtained by updating \(H\) \(m\) times (with \(m\leq k\)) using the inverse Broyden formula \eqref{eq:BroydenInverse} and the pairs \((s_i,y_i)\), \(i=k-m\ldots k-1\).
Then,
\begin{equation}\label{eq:LBroydenInverse}
	H_k
{}={}
	H-(HY-S)\left(M+\trans{S} HY\right)^{-1}\trans{S} H
\end{equation}
where \(S=[s_{k-m},\cdots,s_{k-1}]\), \(Y=[y_{k-m},\cdots,y_{k-1}]\), and
\[
	M_{i,j}
{}={}
	\begin{cases}[@{}l@{~~}l]
		-\innprod{s_{k-m+i}}{s_{k-m+j}} & \text{if } i>j \\[2pt]
		0 & \text{otherwise}
	\end{cases}
\qquad
	i,j=0\ldots m-1.
\]
\end{thm}
Given a vector \(d\in\HH\), computing \(H_kd\) where \(H_k\) is as in \eqref{eq:LBroydenInverse} is very cheap and does not require any matrix inversion, but simply the solution of a small \(m\times m\) linear system.
On the other hand, implementing a limited-memory \emph{modified} Broyden method is trickier than merely replacing \(y_k\) with \(\tilde y_k\).
Indeed, for instance, while in the full modified Broyden \(\vartheta_{k-m}\) was used to enforce some properties on \(H_{k-m+1}\) by means of the relaxed projection
\begin{align*}
	H_{k-m+1}
{}={} &
	\proj_{S_{k-m},\vartheta_{k-m}} H_{k-m},
\shortintertext{the same properties need not hold for \(H_k^1\) by simply letting}
	H_k^1
{}={} &
	\proj_{S_{k-m},\vartheta_{k-m}} H_k^0.
\end{align*}
Each update \(H_k^0\cdots H_k^m=H_{k+1}\) will then require dedicated \(\vartheta_k^0\cdots \vartheta_k^{m-1}\), whence the need of a costly nested-loop recursion as the following (the scheme can clearly be optimized by, \eg storing a buffer of \(\seq{\|s_i\|^2}[i=1][m]\) and temporarily store the scalar products \(\innprod{y_i'}{s_i}\)).
\input{TeX/Alg/Broyden_NestedLoops.tex}%
Matrix \(H_k\) as in \eqref{eq:LBroydenInverse} is well defined as long as the inverse of \(M+\trans{S} HY\) is, in which case it is itself invertible being it derived with the Sherman-Morrison-Woodbury identity \cite{byrd1994representations}.
Consequently, if the selection of \(\vartheta_k\) is made so as to simply enforce nonsingularity, it then makes sense to proceed with the cheap non-modified update \eqref{eq:LBroydenInverse} as long as the \(m\times m\) matrix \(M+\trans{S} HY\) is invertible, and resort to the nested-loop recursion otherwise.



==> TeX/Text/Broyden/LimitedMemory/Restarted.tex <==
In practice, cases in which \eqref{eq:LBroydenInverse} is not well defined occurr extremely rarely, if ever, making the proposed limited-memory variant both robust and efficient.
However, numerical evidence suggests that the use of nonunitary \(\vartheta_k\) can speed up convergence, which on the other hand is discouraged by the computational burden of the nested-loop recursion.
For this reason we propose an efficient \emph{restarted} variant which conforms with the modified Broyden's scheme.
We also allow to perform scalar products in a custom metric \(\innprod\cdot\cdot\) which induces the original \(\innprod\cdot\cdot_\HH\) through the symmetric and positive definite operator \(P\in\linop\), \ie such that \(\innprod\cdot\cdot_\HH=\innprod{\cdot}{P\cdot}\).
This extra option comes in very handy when computing inner products in the Hilbert space \(\HH\) is costly, in which case the custom metric \(\innprod\cdot\cdot\) can be chosen, \eg to be the Euclidean one; otherwise, the original metric can be maintained by simply selecting \(P=\id\).
\begin{algorithm}[ht]
	\algcaption[Restarted modified Broyden method using a single-loop recursion.]{%
		Restarted modified Broyden method in custom metric \(\innprod\cdot\cdot\) using a single-loop recursion.
		\(P\in\linop\) is a symmetric and positive definite operator such that \(\innprod\cdot\cdot_\HH=\innprod{\cdot}{P\cdot}\).%
	}%
	\label{alg:RBroyden}%
	\input{TeX/Alg/RBroyden.tex}%
\end{algorithm}
The procedure is outlined in \Cref{alg:RBroyden}; the scheme requires three memory buffers \(S\) \(\tilde S\) and \(C\), which are initialized as empty and cleared back every time they are full.
\(S\) will contain the last vectors \(Ps_i\), \(\tilde S\) the vectors \(s_i-H_i\tilde y_i\), and \(C\) the scalar products \(\innprod{H_i\tilde y_i}{s_i}_\HH\); if \(\tilde m\in\set{1\ldots m}\) is the size of the current buffer (inclusive of the last pairs \((s_{k-1},y_{k-1})\)), then altogether this requires the storage of \(\tilde m(2n+1)\) scalars.
From the computational point of view, the scheme requires one application of \(P\), two of \(H_k^0\) and \(2n(4\tilde m+1)\) flops (half of which sums and half multiplications).

\Cref{alg:RBroyden} is simply based on reiterations of the relaxed inverse Broyden's update formula \eqref{eq:relaxedInverseBroyden}; at \cref{step:RBroyden:afterLoop} \(\tilde s=H_{k-1}y_{k-1}\) and \(c=\innprod{H_{k-1}y_{k-1}}{s_{k-1}}\), while at \cref{step:RBroyden:tildes} they will be finalized to \(\tilde s=s_{k-1}-H_{k-1}\tilde y_{k-1}\) and \(c=\innprod{H_{k-1}\tilde y_{k-1}}{s_{k-1}}\) thanks to the identities
{\mathloose%
\begin{align*}
	s_{k-1}-H_{k-1}\tilde y_{k-1}
{}={} &
	\theta_{k-1}(s_{k-1}-H_{k-1}y_{k-1})\quad
	\text{and}
\\
	\innprod{s_{k-1}}{H_{k-1}\tilde y_{k-1}}
{}={} &
	(1-\theta_{k-1})\|s_{k-1}\|^2
	{}+{}
	\theta_{k-1}\innprod{s_{k-1}}{H_{k-1}y_{k-1}}.
\end{align*}}%



==> TeX/Text/Broyden/LimitedMemory_Andreas.tex <==
When the problem size is too large even simple linear algebra becomes computationally challenging, not to mention the memory requirements for storing big opesrators.
To overcome the issue, \emph{limited-memory} variants of quasi-Newton schemes exist that use only the last \(m\) couples \((s_k,y_k)\), where \(m\) is a small integer typically between \(3\) and \(20\).
Memory usage is then significantly reduced, and matrix-vector products are replaced by scalar multiplications.
From a theoretical point of view limited-memory quasi-Newton methods cannot be shown to achieve the superlinear convergence rates enjoyed by their full-memory counterparts (cf. \cref{sec:superlinear}).
However, in practice they perform extremely well, oftentimes even beating full-memory methods, and as such are ubiquitous in unconstrained smooth optimization methods.
In \cite{byrd1994representations} an efficient formula tailored for Broyden's method is provided (the extension to Hilbert spaces is straightforward); we restate it here for the reader's convenience.
\begin{thm}[{\cite[Thm. 6.2]{byrd1994representations}}]
Let \(H\in\linop\) be a nonsingular starting operator, and let \(H_k\) be obtained by updating \(H\) \(m\) times (with \(m\leq k\)) using the inverse Broyden formula \eqref{eq:BroydenInverse} and the pairs \((s_i,y_i)\), \(i=k-m\ldots k-1\).
Then,
\begin{equation}\label{eq:LBroydenInverse}
	H_k
{}={}
	H-(HY_k-S_k)\left(M_k+\trans{S_k} HY_k\right)^{-1}\trans{S_k} H
\end{equation}
where \(S_k=[s_{k-m},\cdots,s_{k-1}]\), \(Y_k=[y_{k-m},\cdots,y_{k-1}]\), and
\[
	(M_k)_{i,j}
{}={}
	\begin{cases}[@{}l@{~~}l]
		-\innprod{s_{k-m+i}}{s_{k-m+j}} & \text{if } i>j \\[2pt]
		0 & \text{otherwise}
	\end{cases}
\qquad
	i,j=0\ldots m-1.
\]
\end{thm}
Given a vector \(d\in\HH\), computing \(H_kd\) where \(H_k\) is as in \eqref{eq:LBroydenInverse} is very cheap and does not require any matrix inversion, but simply the solution of a small \(m\times m\) linear system.
On the other hand, implementing a limited-memory \emph{modified} Broyden method is trickier than merely replacing \(y_k\) with \(\tilde y_k\).
Indeed, for instance, while in the full modified Broyden \(\vartheta_{k-m}\) was used to enforce some properties on \(H_{k-m+1}\) by means of the relaxed projection
\begin{align*}
	H_{k-m+1}
{}={} &
	\proj_{S_{k-m},\vartheta_{k-m}} H_{k-m},
\shortintertext{the same properties need not hold for \(H_k^1\) by simply letting}
	H_k^1
{}={} &
	\proj_{S_{k-m},\vartheta_{k-m}} H_k^0.
\end{align*}
Each update \(H_k^0\cdots H_k^m=H_{k+1}\) will then require dedicated \(\vartheta_k^0\cdots \vartheta_k^{m-1}\).
The procedure is summarized in \Cref{alg:LBroyden}, based on the inverse update formula \eqref{eq:BroydenInverse}, where the temporary scalars \(c_i,\nu_i\), \(i=1\ldots m\) are introduced for the sake of avoiding redundant computations.
%The scheme is based on the inverse update formula \eqref{eq:BroydenInverse}, for which
%\[
%	H_kd^k
%{}={}
%	H_{k-1}d^k
%	{}+{}
%	\frac{
%		\innprod{H_{k-1}d}{s_{k-1}}
%	}{
%		\innprod{H_{k-1}y_{k-1}}{s_{k-1}}
%	}
%	\bigl(
%		s_{k-1}-H_{k-1}y_{k-1}
%	\bigr).
%\]
%This can be used to construct operators \(H_k\) using only the last \(m\) couples \((s_j,y_j)\).
%More specifically, starting from an initial invertible operator \(H_k^0\), for \(i=0\ldots m-1\) we let \(H_k^{i+1}\) be the update of \(H_k^i\) using the couple \((s_{k-m+i},y_{k-m+i})\) and set \(H_k=H_k^m\).
%Clearly we shall not compute and store the whole operator \(H_k\), as we are only interested in \(H_kd^k\); however, we will need to compute and temporarily store all the vectors \(y_i'\coloneqq H_k^iy_{k-m+i}\).
\begin{algorithm}[h]
	\algcaption[Modified limited-memory Broyden method using a nested loop recursion.]{%
		Limited memory Broyden method using a nested loop recursion.
	}%
	\label{alg:LBroyden}%
	\input{TeX/Alg/LBroyden.tex}%
\end{algorithm}

One major drawback of \Cref{alg:LBroyden} is the inner loop recursion that requires \(O(m^2)\) scalar products.
%The result in \cite[Thm. 6.2]{byrd1994representations} reduces the complexity to solving a linear system of \(m\) equations, however as long as the non modified Broyden scheme is implemented, \ie for \(\theta_k\equiv 1\).
To overcome this issue, we now propose a \emph{restarted} modified Broyden scheme; differently from the limited-memory version, whenever the buffer of past pairs \((s_k,y_k)\) is full we empty it and restart the scheme.

\begin{algorithm}[h]
	\algcaption[Restarted modified Broyden method using a single-loop recursion.]{%
		Restarted Broyden method using a single-loop recursion.
		Buffers \({\bf s}\), \({\bf y'}\) and \({\bf c}\) contain, respectively, a list of last \(s_i\), \(H_i\tilde y_i\) and \(\innprod{s_i}{H_i\tilde y_i}\).%
	}%
	\label{alg:RBroyden}%
	\input{TeX/Alg/RBroyden.tex}%
\end{algorithm}























==> TeX/Text/Broyden/Relaxation.tex <==
We consider including a relaxation parameter in Broyden's update which shall be tuned in such a way to enforce some wanted properties on Broyden's operators.
In \Cref{subsec:ThetaChoices} we will discuss specific such choices.
In general, given \(\seq{\vartheta_k}\subset[0,2]\) we modify Broyden's update as follows:
\begin{subequations}\label{subeq:Broyden}
\begin{align}
	\label{eq:BroydenB}
	B_{k+1}
{}={} &
	B_k
	{}+{}
	\vartheta_k
	\frac{
		(y_k-B_k s_k)
	}{
		\|s_k\|^2
	}
	{}\otimes{}
	s_k.
\shortintertext{Equivalently, letting \(\tilde y_k=(1-\vartheta_k)B_ks_k + \vartheta_ky_k\),}
	\label{eq:BroydenTilde}
	B_{k+1}
{}={} &
	B_k
	{}+{}
	\frac{
		(\tilde y_k-B_k s_k)
	}{
		\|s_k\|^2
	}
	{}\otimes{}
	s_k
\end{align}
\end{subequations}
resulting in the \emph{relaxed} secant equation
\begin{equation}\label{eq:RelaxedSecant}
	B_{k+1}s_k
{}={}
	\tilde y_k.
\end{equation}
Consequently, \eqref{eq:StandardBroydenProjection} becomes
\begin{equation}\label{eq:BroydenProjection}
	\mathtight
	B_{k+1}
{}={}
	\proj_{\tilde S_k}
	(B_k)
{}={}
	\proj_{S_k,\vartheta_k}
	(B_k)
\qquad\text{where}\quad
	\tilde S_k
{}\coloneqq{}
	\set{B\in\linop}[Bs_k=\tilde y_k].
\end{equation}
We can generalize \eqref{eq:BroydenInverse} to the \emph{relaxed inverse} Broyden's update as follows: letting \(H_k\coloneqq B_k^{-1}\) we have
\begin{equation}\label{eq:relaxedInverseBroyden}
	H_{k+1}
{}={}
	H_k
	{}+{}
	\frac{
		s_k
		{}-{}
		H_k\tilde y_k
	}{
		\innprod{H_k\tilde y_k}{s_k}
	}
	\otimes
	\bigl(
		\trans{H_k}
		s_k
	\bigr).
\end{equation}


==> TeX/Text/Broyden/Restarted_Andreas.tex <==
Letting \(H_k=B_k^{-1}\), for a given direction \(d_k\) from the inverse update formula \eqref{eq:BroydenInverse} we have that
\[
	H_kd_k
{}={}
	H_{k-1}d_k
	{}+{}
	\frac{
		\innprod{H_{k-1}d}{s_{k-1}}
	}{
		\innprod{H_{k-1}y_{k-1}}{s_{k-1}}
	}
	\bigl(
		s_{k-1}-H_{k-1}y_{k-1}
	\bigr).
\]
This can be used to construct operators \(H_k\) using only the last \(m\) couples \((s_j,y_j)\).
More specifically, starting from an initial invertible operator \(H_k^0\), for \(i=0\ldots m-1\) we let \(H_k^{i+1}\) be the update of \(H_k^i\) using the couple \((s_{k-m+i},y_{k-m+i})\) and set \(H_k=H_k^m\).
Clearly we shall not compute and store the whole operator \(H_k\), as we are only interested in \(H_kd_k\); however, we will need to compute and temporarily store all the vectors \(y_i'\coloneqq H_k^iy_{k-m+i}\).


\newpage

On the other hand, implementing a limited-memory \emph{modified} Broyden method is trickier than merely replacing \(y_k\) with \(\tilde y_k\).
Indeed, for instance, while in the full modified Broyden \(\vartheta_{k-m}\) was used to enforce some properties on \(H_{k-m+1}\) by means of the relaxed projection
\[
	H_{k-m+1}
{}={}
	\proj_{S_{k-m},\vartheta_{k-m}} H_{k-m},
\]
the same properties need not hold for \(H_k^1\) by simply letting
\[
	H_k^1
{}={}
	\proj_{S_{k-m},\vartheta_{k-m}} H_k^0.
\]
Each update \(H_k^0\cdots H_k^m=H_{k+1}\) will then require dedicated \(\vartheta_k^0\cdots \vartheta_k^{m-1}\).
The procedure is summarized in \Cref{alg:LBroyden}, where the temporary scalars \(c_i,\nu_i\), \(i=1\ldots m\) are introduced for the sake of avoiding redundant computations.
\begin{algorithm}[h]
	\algcaption[Limited memory Broyden method using a nested loop recursion.]{%
		Limited memory Broyden method using a nested loop recursion.
	}%
	\label{alg:LBroyden}%
	\input{TeX/Alg/LBroyden.tex}%
\end{algorithm}


==> TeX/Text/Broyden/Superlinear.tex <==
From \cite[Thm. 2.2]{dennis1974characterization} and \cite[Thm. 2.1]{more1976global} it follows that the modified Broyden scheme \eqref{subeq:Broyden} with \(\seq{\vartheta_k}\) selected as in \eqref{eq:PowellTheta} satisfies the Dennis-Moré condition \eqref{eq:DM} provided that the mapping whose zeros are sought, \(R\) in our case, is continuously differentiabile around the limiting point, be it \(x_\star\).
In \cite{ip1992local} the requirements for the Dennis-Moré condition to be satisfied for quasi-Newton schemes are relaxed to semidifferentiability around \(x_\star\) and calmness of the semiderivative at \(x_\star\) (cf. \cref{sec:GenDiff}).
For the readers convenience we propose a simplified proof for finite dimensional Hilbert spaces.
\begin{thm}[Broyden's method]\label{thm:BroydenDM}
Suppose that \(\HH\) is finite dimensional and that \(\func F\HH\HH\) is semidifferentiable in a neighborhood \(U_{x_\star}\) of \(x_\star\in\zer F\), the semi\-de\-riv\-a\-tive being calm at \(x_\star\), and let \(G_\star\coloneqq JF(x_\star)\).
Starting from \(x_0\in U_{x_\star}\), let \(\seq{x_k}\) be the sequence recursively defined as in \eqref{eq:xQN} with \(B_k\) given by the modified Broyden's update \eqref{subeq:Broyden} with
\(
	\seq{\vartheta_k}
{}\subset{}
	[\bar\vartheta,2-\bar\vartheta]
\)
for some \(\bar\vartheta>0\).
Suppose the operators \(B_k\) are all nonsingular, and that \(\seq{x_k}\) converges to \(x_\star\) with \(\seq{\|x_k-x_\star\|}\in\ell^1\).

Then, either \(F(x_k)=0\) for some \(k\), or for the Dennis-Moré condition holds
\begin{equation}\label{eq:BroydenDM}
	\lim_{k\to\infty}{
		\frac{
			\|(B_k-G_\star)s_k\|
		}{
			\|s_k\|
		}
	}
{}={}
	0.
\end{equation}
\begin{proof}
See \Cref{proof:thm:BroydenDM}.
\end{proof}
\end{thm}

\begin{rem}\label{rem:Broydenw}
It is evident from its proof that \Cref{thm:BroydenDM} remains valid if \(\seq{B_k}\) is updated using \(s_k=w_k-x_k\) and \(y_k=Fw_k-Fx_k\), where \(\seq{w_k}\) is an arbitrary sequence such that
\(
	\seq{\|w_k-x_\star\|}
{}\in{}
	\ell^1
\).
To see this, simply trace the proof of \Cref{thm:BroydenDM} replacing any occurrence of \(x_k\) with \(w_k\), yet leaving those of \(x_{k+1}\) unchanged.
\end{rem}


%\begin{thm}[{Superlinear convergence of the \refSM[] with relaxed Broyden's method}]\label{thm:SuperMannBroyden}
%Suppose that \(\HH\) is finite dimensional and let \(\func T\HH\HH\) be an \avg{} operator for some \(\alpha\in(0,1]\), with \(\fix T\neq\emptyset\).
%Let \(R\coloneqq\id-T\) and let \(\seq{x_k}\) be the sequence generated by the \refSM{}, \(\seq{\varepsilon_k}\) \(Q\)-linearly convergent to \(0\), and \(d_k=B_k^{-1}Rx_k\) for all \(k\), \(\seq{B_k}\) being chosen according to the modified Broyden's scheme of \Cref{subsec:ThetaChoices} with
%\[
%	s_k=w_k-x_k
%\qquad\text{and}\qquad
%	y_k=Rw_k-Rx_k
%\]
%starting from an invertible operator \(B_0\in\linop\).
%Suppose that \(\seq{B_k^{-1}}\) remains bounded, and that \(R\) is calmly semidifferentiable and metrically subregular at the limit \(x_\star\) of \(\seq{x_k}\).

%Then, \(\seq{d_k}\) satisfies \eqref{eq:DM}, \ie, the directions are superlinearly convergent, and all the claims of \Cref{thm:Local} hold.
%In particular \(\seq{\|Rx_k\|}\) converges \(Q\)-superlinearly and both \(\seq{x_k}\) and \(\seq{\dist(x_k,\fix T)}\)~ \(R\)-superlinearly.
%\begin{proof}
%See \Cref{proof:thm:SuperMannBroyden}.
%\end{proof}
%\end{thm}






==> TeX/Text/Broyden/ThetaChoices.tex <==
















==> TeX/Text/Broyden/ThetaChoices/Nonsingularity.tex <==
From the rank-one update determinant formula
\[
	\det(A+u\otimes v)
{}={}
	\bigl(1+\innprod{v}{A^{-1}u}\bigr)
	\det A
\]
we obtain
\[
	\det B_{k+1}
{}={}
	(1+(\gamma_k-1)\vartheta_k)
	\det B_k
\quad\text{where}\quad
	\gamma_k
{}\coloneqq{}
	\tfrac{1}{\|s_k\|^2}
	\innprod{s_k}{B_k^{-1}y_k}.
\]
Enforcing \(|\det B_{k+1}|\geq\bar\vartheta|\det B_k|\) for some \(\bar\vartheta\in(0,1)\) amounts to selecting \(\vartheta_k\in[0,2]\) such that
\(
	\bigl|1+(\gamma_k-1)\vartheta_k\bigr|
{}\geq{}
	\bar\vartheta
\),
\ie
\begin{equation}\label{eq:thetaInvertible}
	\begin{cases}[rl@{\quad}l]
		\vartheta_k & {}\in{} [0,2] & \text{if } \gamma_k\geq 1 \\
		\vartheta_k & {}\in{}
			\bigl[
				0,
				\tfrac{1-\bar\vartheta}{1-\gamma_k}
			\bigr] \cup \bigl[
				\tfrac{1+\bar\vartheta}{1-\gamma_k},
				2
			\bigr] & \text{if } \gamma_k<1.
	\end{cases}
\end{equation}
\cite{powell1970numerical} selects the \(\vartheta_k\) closest to \(1\) that satisfies \eqref{eq:thetaInvertible}, namely
\begin{equation}\label{eq:PowellTheta}
	\vartheta_k
{}\coloneqq{}
	\begin{cases}[l@{~~\text{if }}l]
			1
		&
			|\gamma_k| \geq \bar\vartheta
		\\
			\frac{
				1-\sgn(\gamma_k)
				\bar\vartheta
			}{
				1-\gamma_k
			}
		&
			|\gamma_k| < \bar\vartheta
	\end{cases}
\end{equation}
with the convention \(\sgn 0=1\).
This also ensures
\(
	|1-\vartheta_k|
{}\leq{}
	\bar\vartheta
\).


==> TeX/Text/Broyden/ThetaChoices/PositiveCurvature.tex <==
If the mapping \(F\) is monotone, \ie such that
\(
	\innprod{Fy-Fx}{y-x}\geq 0
\)
for any \(x,y\in\HH\) and \(F\) is (semi)differentiable at \(x\), then
\[
	0
{}\leq{}
	\innprod{Fy-Fx}{y-x}
{}={}
	\innprod{JF(x)(y-x)}{y-x}
	{}+{}
	o(\|y-x\|^2).
\]
When close to a nonsingular solution, the quantity above is strictly positive, and since \(B_{k+1}s_k\) should approximate \(JF(x_k)s_k\) it makes sense to enforce a positive curvature condition.
\begin{lem}\label{prop:thetaPosCurv}
Consider the modified Broyden's update \eqref{subeq:Broyden} for a monotone \(F\).
Fix \(\alpha\in(0,1)\) and let \(\delta_k\coloneqq\innprod{B_ks_k}{s_k}\).
The \(\vartheta_k\in[0,2]\) for which
\begin{subequations}
\begin{equation}\label{eq:thetaPosCurv}
	\innprod{B_{k+1}s_k}{s_k}
{}\geq{}
	\alpha\bigl|\innprod{B_ks_k}{s_k}\bigr|
\end{equation}
are exactly
\begin{equation}
	\begin{cases}[rl@{\quad}l]
		\vartheta_k & {}\in{}
			\left[
				0,
				\frac{(1-\alpha)\delta_k}{\delta_k-\innprod{y_k}{s_k}}
			\right] & \text{if }~ \frac{2\innprod{y_k}{s_k}}{1+\alpha}<\delta_k
	\\[5pt]
		\vartheta_k & {}\in{}
			\left[
				\frac{(1+\alpha)\delta_k}{\delta_k-\innprod{y_k}{s_k}},
				2
			\right] & \text{if }~ \delta_k<0
	\\[5pt]
		\vartheta_k & {}\in{}
			\left[
				0,2
				\vphantom{\frac{\delta_k}{\delta_k}}
			\right] & \text{otherwise}
	\end{cases}
\end{equation}
In particular, the closest to \(1\) is
\begin{equation}
	\vartheta_k
{}={}
	\begin{cases}[l@\quad l]
		1 & \text{if }~ \alpha|\delta_k|\leq\innprod{y_k}{s_k}\\
		\frac{1-\alpha\sgn(\delta_k)}{\delta_k-\innprod{y_k}{s_k}}\delta_k & \text{otherwise.}
	\end{cases}
\end{equation}
\end{subequations}
\begin{proof}
Since
\(
	B_{k+1}s_k
{}={}
	\tilde y_k
{}={}
	(1-\vartheta_k)B_ks_k+\vartheta_ky_k
\),
condition \eqref{eq:thetaPosCurv} can be rewritten as
\(
	(1-\vartheta_k)\delta_k
	{}+{}
	\vartheta_k\innprod{y_k}{s_k}
{}\geq{}
	\alpha|\delta_k|
\),
\ie
\[
	\vartheta_k(\innprod{y_k}{s_k}-\delta_k)
{}\geq{}
	\alpha|\delta_k|-\delta_k.
\]
\begin{itemize}
	\item
		If \(\delta_k=\innprod{y_k}{s_k}\) then any value of \(\vartheta_k\in[0,2]\) is acceptable.
		Indeed,
		\(
			\alpha|\delta_k|-\delta_k\leq -(1-\alpha)\delta_k=-(1-\alpha)\innprod{y_k}{s_k}
		\)
		which is negative, due to the fact that \(\innprod{y_k}{s_k}\geq 0\) by monotonicity.
	\item
		If \(\delta_k>\innprod{y_k}{s_k}\geq 0\), then
		\[
			\vartheta_k
		{}\leq{}
			\frac{
				\alpha|\delta_k|-\delta_k
			}{
				\innprod{y_k}{s_k}-\delta_k
			}
		{}={}
			\frac{
				(1-\alpha)\delta_k
			}{
				\delta_k-\innprod{y_k}{s_k}
			},
		\]
		which admits feasible values of \(\vartheta_k\) since the right-hand side is at least \(1-\alpha\).
		Moreover, for \(\delta_k\leq\frac{2\innprod{y_k}{s_k}}{1+\alpha}\) the right-hand side is larger than \(2\), and as such any \(\vartheta_k\in[0,2]\) is feasible.
	\item
		If \(\delta_k<\innprod{y_k}{s_k}\), then
		\[
			\vartheta_k
		{}\geq{}
			\frac{
				\alpha|\delta_k|-\delta_k
			}{
				\innprod{y_k}{s_k}-\delta_k
			}.
		\]
		If \(\delta_k\geq 0\), then any value of \(\vartheta_k\in[0,2]\) is acceptable.
		Otherwise,
		\[
			\vartheta_k
		{}\geq{}
			\frac{
				(1+\alpha)|\delta_k|
			}{
				\innprod{y_k}{s_k}+|\delta_k|
			}
		\]
		which always admits feasible \(\vartheta_k\in[0,2]\) since the right-hand side is at most \(1+\alpha\).\qedhere
\end{itemize}
\end{proof}
\end{lem}
If the \(x\)-update rule is \(w_k=x_k-\tau_kB_k^{-1}Fx_k\), so that \(s_k=w_k-x_k\), then the inverse Broyden update \eqref{eq:BroydenInverse} will reasonably be performed rather than \eqref{subeq:Broyden}.
Here, consistently with the \refSM[] we allow for an intermediate step \(w_k\) in between \(x_k\) and \(x_{k+1}\); clearly, \(w_k=x_{k+1}\) is a feasible choice.
The quantity \(\delta_k=\innprod{B_ks_k}{s_k}\) can be retrieved thanks to the identity \(s_k=-\tau_kB_k^{-1}Fx_k\) which results in
\begin{equation}\label{eq:delta_k}
	\delta_k
{}={}
	-\tau_k\innprod{Fx_k}{s_k}.
\end{equation}


\begin{rem}[Nonsingularity \textit\& positive curvature]
From \eqref{eq:thetaInvertible} and \Cref{prop:thetaPosCurv} it follows that if \(F\) is monotone, then for any \(\alpha,\bar\vartheta\in(0,1)\) it is always possible to find \(\vartheta_k\) with \(|1-\vartheta_k|\leq\max\set{\alpha,\bar\vartheta}\) such that the modified Broyden's update \eqref{subeq:Broyden} satisfies
\[
	\bigl|\det B_{k+1}\bigr|
{}\geq{}
	\bar\vartheta\bigl|\det B_k\bigr|
\quad\text{and}\quad
	\innprod{B_{k+1}s_k}{s_k}
{}\geq{}
	\bigl|\innprod{B_ks_k}{s_k}\bigr|.
\]
In particular, letting
\(
	\gamma_k
{}={}
	\frac{
		\innprod{B_k^{-1}y_k}{s_k}
	}{
		\|s_k\|^2
	}
\),~
\(
	\delta_k
{}={}
	\innprod{B_ks_k}{s_k}
\),~
and \(\sigma_k=\sgn\delta_k\), the \(\vartheta_k\) closest to \(1\) can be selected with the following scheme:
\input{TeX/Alg/thetaChoice.tex}\let\qed\relax%
\end{rem}



==> TeX/Text/Definitions/Differentiability.tex <==
Recall that \(\func F\HH\HH\) is \DEF{differentiable} at \(\bar x\) if there exists \(JF(\bar x)\in\linop\) such that
\[
	\lim_{
		\substack{x\to\bar x\\x\neq\bar x}
	}{
		\frac{
			Fx-F\bar x-JF(\bar x)(x-\bar x)
		}{
			\|x-\bar x\|
		}
	}
{}={}
	0.
\]
In such case, \(JF(\bar x)\) is unique and is the \DEF{Jacobian} of \(F\) at \(\bar x\).
The next result follows straightforwardly from the definition of differentiability.
\begin{lem}\label{lem:JStronglyNonsingular}
Suppose that \(\func F\HH\HH\) is differentiable at \(\bar x\) and \(JF(\bar x)\in\linop\) is strongly nonsingular.
Then, there exist two constants \(\varepsilon,\gamma>0\) such that
\[
	\|Fx-F\bar x\|
{}\geq{}
	\gamma\|x-\bar x\|
\qquad
	\forall x\in B(x,\varepsilon).
\]
\end{lem}
We now list some different notions of differentiability which will be needed later on in the paper.
%We remind that an operator \(\func F\HH\HH\) is \DEF{calm} at \(\bar x\in\HH\) if there exists a neighborhood \(U_{x_\star}\) of \(x_\star\) and a constant \(L_F\geq 0\) such that
\(
	\|Fx-F\bar x\|
{}\leq{}
	L_F\|x-\bar x\|
\)
for all \(x\in U_{x_\star}\).
\begin{defin}[Semiderivative]
We say that an operator \(\func F\HH\HH\) is \DEF{semidifferentiable} at \(\bar x\) if there exists a continuous and positively homogeneous function
\(
	\func{\Bjac F{\bar x}}{\HH}{\HH}
\),
called the \DEF{semiderivative} of \(F\) at \(\bar x\), such that
\[
	F(x)
{}={}
	F(\bar x)
	{}+{}
	\Bjac F{\bar x}[x-\bar x]
	{}+{}
	o(\|x-\bar x\|).
\]
The semiderivative is (\DEF{Lipschitz-})\DEF{continuous} at \(\bar x\) if the function \(x\mapsto\Bjac Fx[w]\) is (Lipschitz-)continuous at \(\bar x\) for all \(w\in\HH\).
\end{defin}
By positive homogeneity, (Lipschitz-)continuity of \(x\mapsto\Bjac Fx[w]\) for all \(w\in\HH\) is equivalent to that for all \(w\in\HH\) with \(\|w\|=1\).
Semidifferentiability is clearly a milder property than differentiability in that the mapping \(\Bjac F{\bar x}\) needs not be linear; the interested reader is referred to \cite[§7]{rockafellar2011variational} for an extensive discussion.
When \(F\) is strictly continuous (\ie locally Lipschitz continuous) at \(\bar x\), semidifferentiability at \(\bar x\) is equivalent to directional differentiability at \(\bar x\) \cite[Prop. 3.1.3]{facchinei2003finite} and the semiderivative is sometimes rather called \emph{\(B\)-derivative} (see e.g. \cite{pang1990newtons,ip1992local,facchinei2003finite}).
\begin{defin}[Strict differentiability]
We say that \(\func F\HH\HH\) is \DEF{strictly differentiable} at \(\bar x\) if it is differentiable there and the \DEF{Jacobian} matrix \(JF(\bar x)\) of \(F\) at \(\bar x\) satisfies
\begin{equation}\label{eq:StrictDiff}
	\lim_{%
		\substack{(y,z)\to(\bar x,\bar x)\\y\neq z}
	}{
		\frac{
			\left\|
				F(y)-F(x)-JF(\bar x)(y-x) 
			\right\|
		}{
			\|y-x\|
		}
	}
{}={}
	0.
\end{equation}
\end{defin}
There is a slight ambiguity in the literature, whereas such property is sometimes referred to as \emph{strong} (see e.g. \cite{pang1990newtons,ip1992local}) rather than \emph{strict} differentiability.
We stick to the proposed notation which is taken from \cite{rockafellar2011variational}.
%and we will consider the following notion of \emph{strong} differentiability.
%\begin{defin}[Strong differentiability]
%We say that \(\func{F}{\F^n}{\F^m}\) is \DEF{strongly differentiable} at \(\bar x\) if it is differentiable there and the \DEF{Jacobian} matrix \(JF(\bar x)\) of \(F\) at \(\bar x\) satisfies
%\begin{equation}\label{eq:StrongDiff}
%	\limsup_{%
%		\substack{(y,z)\to(\bar x,\bar x)\\y\neq z}
%	}{
%		\frac{
%			\left\|
%				F(y)-F(x)-JF(\bar x)(y-x) 
%			\right\|
%		}{
%			\|y-x\|^2
%		}
%	}
%{}<{}
%	\infty
%\end{equation}
%\end{defin}

%{\color{red}
%\begin{thm}
%Suppose that \(\func{F}{\F^n}{\F^m}\) is \DEF{strongly differentiable} at \(\bar x\), then \(F\) is calm at \(\bar x\).
%\end{thm}
%}%

%\begin{thm}
%Let \(\func{F}{\F^n}{\F}\).
%Then, the following hold:
%\begin{enumerate}
%	\item\label{item:DiffSemidiff} if \(F\) is differentiable at \(\bar x\) then it is also semidifferentiable at \(\bar x\) with \(\Bjac F{\bar x}=JF(\bar x)\);
%	\item\label{item:StrictDiff} \(F\) is strictly differentiable at \(\bar x\) iff it is continuously semidifferentiable at \(\bar x\);
%%	\item\label{item:JNonsingular} if \(F\) is strictly differentiable at \(\bar x\) and \(JF(\bar x)\) is nonsingular, then there exist \(\rho>0\) and a neighborhood \(U_{\bar x}\) of \(\bar x\) such that
%%		\[
%%			\|F(y)-F(z)\|
%%		{}\geq{}
%%			\rho\|y-z\|
%%		\qquad
%%			\forall y,z\in U_{\bar x}
%%		\]
%	\item\label{item:SemiCalm} if \(\Bjac F{\cdot}\) is \emph{calm} at \(\bar x\) with modulus \(L\) in a neighborhood \(U_{\bar x}\) of \(\bar x\),%
%		\footnote{Calmness is equivalent to Lipschitz continuity \emph{at} one point;
%			more precisely, we say that \(F\) is \DEF{calm} with modulus \(L\) at \(\bar x\) in \(U\) if for all \(x\in U\) it holds that \(\|F(x)-F(\bar x)\|\leq L\|x-\bar x\|\).}
%		then
%		\[
%			\frac{
%				|F(y)-F(z)|
%			}{
%				\|y-z\|
%			}
%		{}\leq{}
%			L
%			\max
%			\set{
%				\|y-\bar x\|
%				{},{}
%				\|z-\bar x\|
%			}
%		\qquad
%			\forall y,z\in U_{\bar x}
%			,~~
%			y\neq z
%		\]
%\end{enumerate}
%\begin{proof}
%\ref{item:DiffSemidiff} is obvious from the definition of semidifferentiability, \ref{item:StrictDiff} is shown in \cite[Thm. 7.21(e)]{rockafellar2011variational},
%%then \ref{item:JNonsingular} follows from \cite[Lem. 2.2]{ip1992local}
%and finally \ref{item:SemiCalm} from \cite[Lem. 2.2]{ip1992local} by observing that the proof works even assuming calmness in place of Lipschitz continuity.
%\end{proof}
%\end{thm}
	







==> TeX/Text/Definitions/GenDiff.tex <==
For the reader's convenience we list some known result for semidifferentiable functions which are proven in the literature for functions in \(\R^n\), but whose proofs straightforwardly extend to Hilbert spaces.
Recall that \(\func F\HH\HH\) is \DEF{differentiable} at \(\bar x\) if there exists \(\jac F{\bar x}\in\linop\) such that
\[
	\lim_{
		\substack{x\to\bar x\\x\neq\bar x}
	}{
		\frac{
			Fx-F\bar x-\jac F{\bar x}(x-\bar x)
		}{
			\|x-\bar x\|
		}
	}
{}={}
	0.
\]
In such case, \(\jac F{\bar x}\) is unique and is the \DEF{Jacobian} of \(F\) at \(\bar x\).
%The next result follows straightforwardly from the definition of differentiability.
%\begin{lem}\label{lem:JStronglyNonsingular}
%Suppose that \(\func F\HH\HH\) is differentiable at \(\bar x\) and \(\jac F{\bar x}\in\linop\) is strongly nonsingular.
%Then, there exist two constants \(\varepsilon,\gamma>0\) such that
%\[
%	\|Fx-F\bar x\|
%{}\geq{}
%	\gamma\|x-\bar x\|
%\qquad
%	\forall x\in B(x,\varepsilon).
%\]
%\end{lem}
We say that \(\func F\HH\HH\) is \DEF{calm} at \(\bar x\in\HH\) if there exist a neighborhood \(U_{x_\star}\) of \(x_\star\) and a constant \(L_F\geq 0\) such that
\(
	\|Fx-F\bar x\|
{}\leq{}
	L_F\|x-\bar x\|
\)
for all \(x\in U_{x_\star}\).
Calmness is somewhere referred to as Lipschitz continuity \emph{at} one point.

\begin{defin}[Strict differentiability]\label{defin:semidiff}
We say that \(\func F\HH\HH\) is \DEF{strictly differentiable} at \(\bar x\) if it is differentiable there with \(\jac F{\bar x}\) satisfying
\begin{equation}\label{eq:StrictDiff}
	\lim_{%
		\substack{(y,z)\to(\bar x,\bar x)\\y\neq z}
	}{
		\frac{
			\left\|
				Fy-Fx-\jac F{\bar x}(y-x) 
			\right\|
		}{
			\|y-x\|
		}
	}
{}={}
	0.
\end{equation}
\end{defin}
There is a slight ambiguity in the literature, whereas such property is sometimes referred to as \emph{strong} (see e.g. \cite{pang1990newtons,ip1992local}) rather than \emph{strict} differentiability.
We stick to the proposed notation which is taken from \cite{rockafellar2011variational}.

\begin{defin}[Semiderivative]
We say that an operator \(\func F\HH\HH\) is \DEF{semidifferentiable} at \(\bar x\) if there exists a continuous and positively homogeneous function
\(
	\func{\Bjac F{\bar x}}{\HH}{\HH}
\),
called the \DEF{semiderivative} of \(F\) at \(\bar x\), such that
\[
	Fx
{}={}
	F\bar x
	{}+{}
	\Bjac F{\bar x}[x-\bar x]
	{}+{}
	o(\|x-\bar x\|).
\]
We say that the semiderivative is \DEF{continuous} (resp. (\DEF{calm})) at \(\bar x\) if the function \(x\mapsto\Bjac Fx[w]\) is continuous (resp. calm) at \(\bar x\) for all \(w\in\HH\).
\DEF{Strict semidifferentiability} is defined as in \Cref{defin:semidiff}.
\end{defin}
By positive homogeneity, continuity and/or calmness of \(x\mapsto\Bjac Fx[w]\) for all \(w\in\HH\) is equivalent to that for all \(w\in\HH\) with \(\|w\|=1\).
Semidifferentiability is clearly a milder property than differentiability in that the mapping \(\Bjac F{\bar x}\) needs not be linear; the interested reader is referred to \cite[§7]{rockafellar2011variational} for an extensive discussion.
When \(F\) is strictly continuous (\ie locally Lipschitz continuous) at \(\bar x\), semidifferentiability at \(\bar x\) is equivalent to directional differentiability at \(\bar x\) \cite[Prop. 3.1.3]{facchinei2003finite} and the semiderivative is sometimes rather called \emph{\(B\)-derivative} (see e.g. \cite{pang1990newtons,ip1992local,facchinei2003finite}).











==> TeX/Text/GenMann/Comparisons.tex <==
GKM iterations are in the same flavor of the updates in \cite[Alg. 2.1]{solodov1998globally}.
%\cite[Alg. 5.32]{izmailov2014newton}
The cited scheme solves \eqref{eq:Problem} where \(R\) is a continuous monotone operator, not necessarily the residual of a nonexpansive one.
\Cref{alg:SS} translates it into our framework, where \(R\) is instead the residual of a FNE operator \(T\).
The parameter \(\sigma_k>0\) depends on the positive definite matrix \(B_k\) in such a way that the line search \eqref{eq:SS-LS} is feasible.
\begin{algorithm}[H]
	\algcaption{Solodov \& Svaiter's {\cite[Alg. 2.1]{solodov1998globally}}. \emph{(Exact) Globalized Newton Method for Monotone Equations}}%
	\label{alg:SS}%
	\input{TeX/Alg/SS.tex}
\end{algorithm}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[tb]
	\setlength\fboxsep{0pt}%
	\fbox{%
		\begin{minipage}[t]{0.33\textwidth}%
			\vspace*{0pt}%
			\includetikz[width=\linewidth]{IS1}%
		\end{minipage}%
	}%
	\hfill
	\fbox{%
		\begin{minipage}[t]{0.33\textwidth}%
			\vspace*{0pt}%
			\includetikz[width=\linewidth]{IS2}%
		\end{minipage}%
	}%
	\hfill
	\fbox{%
		\begin{minipage}[t]{0.33\textwidth}%
			\vspace*{0pt}%
			\includetikz[width=\linewidth]{IS3}%
		\end{minipage}%
	}%
	\caption[Comparison between GKM and S\&S updates]{%
		The \emph{descent condition} \eqref{eq:SS-LS} prevents the update directions \(d^k\) in S\&S's scheme to point in the gray-shaded area.
		As a result, differently from the GKM scheme, S\&S is not robust to any choice of direction and cannot accept for instance the (bad) direction as in \Cref{fig:SuperMann}.
		In any case, the half-space \(C_w\) onto which \(x\) is projected according to the GKM scheme is properly contained in the half-space \(H_w\) corresponding to the S\&S's update.
		As a result, the GKM update is always closer than S\&S's to the set of solutions.
	}%
	\label{fig:SS}%
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{rem}[Half-spaces in S\&S and GKM]
	Denoting \(C_k=C_{w^k}\) as in \cref{lem:DriftedKM} so that \(x^{k+1}=\proj_{C_k}x^k\) in the GKM scheme (where for simplicity we choose \(\lambda_k=1\) and \(\mu_k=0\)), for the half-spaces \eqref{eq:SS-Hk} it holds that
	\[
		\zer R\subseteq C_k\subseteq H_k,
	\]
	the last inclusion holding as equality iff \(Rw^k=0\).
	This means that in the GKM scheme, the same \(w^k\) yields an iterate \(x^{k+1}\) which is closer to \(\zer R\) with respect to S\&S's update (cf. \Cref{fig:SS}).
	Notice further that the hyperplanes delimiting the two half-spaces are parallel, with \(\partial C_k\) passing by \(Tw^k\) and \(\partial H_k\) by \(w^k\).
\end{rem}
\begin{rem}[Directions in S\&S and GKM]
	Solodov \& Svaiter impose specific choices for the direction \(d^k\) (cf. \Cref{fig:SS}) which is due to the fact that they address a broader class of operators for which the geometrical properties that led to the GKM scheme do not apply.
	Because of our specialization to FNE operators (recall that we always reduce to the case of FNE operators through the suitable \(\nicefrac{1}{2\alpha}\)\,-averaging), we instead have complete freedom in selecting \(d^k\).
	\Cref{alg:SS} in its extended version allows for a range of inexactness in computing \(d^k\), however our scheme is robust to \emph{any} error.
\end{rem}



==> TeX/Text/GenMann/Convergence.tex <==
We now show how iterating GKM steps gives rise to an algorithm that extends the KM scheme and mantains the same convergence properties.
To rule out trivialities, in the following we assume that a solution to \eqref{eq:Problem} is not found in a finite number of iterations, so that \(\|Rx_k\|\neq 0\) and \(\|Rw_k\|=0\) for all \(k\).
\begin{thm}[GKM scheme]\label{thm:GKM}
Let
\(\beta,\sigma\in(0,1)\),
\(x_0\in\HH\),
\(\seq{\lambda_k}\subset[0,\nicefrac1\alpha]\),
and \(\seq{d_k}\subset\HH\) be fixed.
Starting from \(k=0\), consider the iterates generated by the generalized KM scheme (GKM)

\boxedalgorithmic[\small\normalfont\sf]{%
	\STATE{%
		\(
			w_k
		{}={}
			x_k+\tau_kd_k
		\)

		where \(\tau_k=\beta^{i_k}\), and \(i_k\in\N\) is the smallest such that
		\[
			\rho_k
		{}\coloneqq{}
			\|Rw_k\|^2
			{}-{}
			2\alpha
			\innprod{Rw_k}{w_k-x_k}
		{}\geq{}
			\sigma
			\|Rw_k\|
			\|Rx_k\|
		\]
	}%
	\label{state:GKM:initial}%
	\STATE{%
		\vspace{-0.75\baselineskip}%
		\(
			x_{k+1}
		{}={}
			x_k
			{}-{}
			\lambda_k
			\frac{\rho_k}{\|Rw_k\|^2}Rw_k
		\)%
	}%
	\STATE{%
		set \(k\gets k+1\) and go to \cref{state:GKM:initial}.
	}%
}

Then,
\begin{enumerate}
	\item\label{thm:GKM:Fejer}\(\seq{x_k}\) is Fejér monotone with respect to \(\fix T\), with
		\[
			\|x_{k+1}-z\|^2
		{}\leq{}
			\|x_k-z\|^2
			{}-{}
			\sigma^2
			\lambda_k(\nicefrac1\alpha-\lambda_k)
			\|Rx_k\|^2
		\quad
			\forall z\in\fix T;
		\]
	\item\label{thm:GKM:Tau_k}
		for all \(k\in\N\), \(\tau_k=1\) if \(d_k=0\), and
		\(
			\tau_k
		{}\geq{}
			\min\set{
				\beta\frac{1-\sigma}{4\alpha\|d_k\|}
				{},{}
				1
			}
		\)
		otherwise.
\end{enumerate}
Moreover, if
\(
	\seq{\lambda_k}\subset[\delta,\nicefrac1\alpha-\delta]
\)
for some \(\delta>0\), then the following also hold:
\begin{enumerate}[resume]
	\item\label{thm:GKM:ResStr}
		\(Rx_k\to 0\) with \(\seq{\|Rx_k\|}\in\ell^2\);
	\item\label{thm:GKM:xWeak}
		\(\seq{x_k}\) converges weakly to a point \(x_\star\in\fix T\).
\end{enumerate}
If additionally \(\seq{x_k}\) converges strongly to a point \(x_\star\) (this being true if \(\HH\) is finite dimensional) at which \(R\) is metric subregular, then
\begin{enumerate}[resume]
	\item\label{thm:GKM:Linear}
		\(\|Rx_k\|\to 0\)~ \(R\)-linearly and \(\dist(x_k,\fix T)\to 0\)~ \(Q\)-linearly;
	\item\label{thm:GKM:xLinear}
		if there exists a constant \(D\geq 0\) such that \(\|d_k\|\leq D\|Rx_k\|\), then \(x_k\to x_\star\)~ \(R\)-linearly.
\end{enumerate}
\begin{proof}
See \Cref{proof:thm:GKM}.
\end{proof}
\end{thm}


%\begin{rem}
%If \(\HH\) is infinite dimensional only weak convergence of the sequence is ensured.
%However, as it holds for the classical KM scheme, because of Fejér monotonicity if \(R\) is metrically subregular at the weak limit \(x_\star\) with radius, say, \(\varepsilon\), then strong convergence holds as long as \(x_{\bar k}\) gets \(\varepsilon\)-close to \(x_\star\) for some \(\bar k\).
%\end{rem}







==> TeX/Text/General/Generalizations.tex <==
Though already quite broad and not restrictive, some hypotheses of \Cref{thm:General:Global} can be further relaxed without affecting the validity of the result.
To avoid further complicating the framework we intentionally defer these minor details in the following side remarks.
\begin{rem}[\emph{Quasi-}Fejér safeguard updates]
All claims in \cref{{thm:General:Global},{prop:K0K1}} remain valid if the Fejér condition \eqref{eq:General:K2} that characterizes safeguard updates at step \ref{step:General:K2} is relaxed to quasi-Fejér monotonicity.
Namely, it can be replaced by
\[
	\|x_{k+1}-z\|^2
{}\leq{}
	\|x_k-z\|^2
	{}-{}
	\sigma\|Rx_k\|^2
	{}+{}
	\varepsilon_k(z)
\quad
	\forall z\in\fix T
\]
where for all \(z\in\fix T\) \(\seq{\varepsilon_k(z)}\in\ell_+^1\) is a summable sequence.

For \cref{thm:General:Summable} to hold too, it can be easily verified that it suffices to restrict \(\seq{\varepsilon_k(z)}\in\ell_+^{\nicefrac12}\) for all \(z\in\fix T\); in fact, \eqref{eq:K2linear} becomes
\[
	\|x_{k+1}-z_{k+1}\|
{}\leq{}
	\rho\|x_k-z_k\|
	{}+{}
	{\textstyle\sqrt{\varepsilon_k(z_k)}}
\qquad
	\forall k\in K_2,~\geq\bar k,
\]
and the rest of the proof easily follows, since due to strong convergence (hence boundedness) of the ``shadow sequence'' \(\seq{z_k}\) \cite[Prop. 3.5(b)]{combettes2001quasi} we may omit the dependency of \(z_k\) in the error \(\varepsilon_k\).

With the same reasoning, \cref{thm:General:Linear} still holds as long as the error \(\seq{\varepsilon_k(z)}\) is linearly convergent for all \(z\in\fix T\).
\end{rem}
%\begin{rem}[No need for \eqref{eq:D} for safeguard steps \ref{step:General:K2}]\label{rem:DK2}
%\hl{Really? Probably some problems with linear convergence. In any case who cares, as in SuperMann this is ensured (write it explicitely!)}
%The fact that \(x_{k+1}\) is not too far from \(x_k\) ensures that the distance from \(\fix T\) and the residual do not grow too much in between iterations (cf. \eqref{eq:K+1z} and \eqref{eq:Rk+1}).
%However, these properties are only used for \ref{K0}- and \ref{K1}-updates, specifically in \eqref{eq:D1}, \eqref{eq:D2} and \eqref{eq:D3} (in this last one observe that \(\gamma_2(k)-1\notin K_2\)).
%Therefore, \emph{\Cref{thm:General:Global} remains valid if \eqref{eq:D} is only required for \(k\in K_0\cup K_1\), \ie, for iterates passing the test at either step \ref{step:General:K0} or \ref{step:General:K1}}.
%\end{rem}
%
%\begin{rem}[Less conservative \(r_{\rm safe}\) for step \ref{step:General:K1}]\label{rem:r_safeK2}
%As anticipated, the parameter \(r_{\rm safe}\) is needed only to control the transition from \ref{K2}- to \ref{K1}-updates.
%This is evident from the proof of \Cref{thm:General:Global}, where \(r_{\rm safe}\) is only used in \eqref{eq:r_safe}, and since one among \(K_0\) and \(K_1\) is required to be empty in the proof of linear convergence.
%\emph{To favor \ref{K1}-updates we may therefore set \(r_{\rm safe}\gets\infty\) after every \ref{K0}-update at step \ref{step:General:K0}} (there is no need to do so also after \ref{K1}-updates).
%\end{rem}
%\begin{rem}[Omitting \(r_{\rm safe}\) for monotone \emph{safeguard} updates]
%In light of \Cref{rem:r_safeK2}, if the \emph{safeguard} updates in step \ref{step:General:K2} are such that \(\|Rx_{k+1}\|\leq\|Rx_k\|\), then the parameter \(r_{\rm safe}\) plays no role and can be omitted.
%\end{rem}
%
%\begin{rem}[Variable \(\sigma\)'s for the safeguard step \ref{step:General:K2}]\label{rem:sigma_k}
%\emph{With the only exception of \ref{thm:General:Summable}, all the other claims of \Cref{thm:General} still hold if in condition \eqref{eq:General:K2} the constant \(\sigma\) at each iteration \(k\) is replaced by any \(\sigma_k\geq0\), as long as \(\seq{\sigma_k}\notin\ell^1\)}.
%Indeed, \eqref{eq:sigmaConstant} with variable \(\sigma_k\)'s becomes
%\[
%	\|x_0-z\|^2
%{}\geq{}
%	\sum_{k\in K_2}{
%		\bigl(
%			\sigma_k
%			\|Rx_k\|^2
%			{}-{}
%			\varepsilon_k(z)
%		\bigr)
%	}
%	~{}-{}~~
%	\sum_{\mathclap{k\in K_0\cup K_1}}\varepsilon_k'(z).
%\]
%and square-summability of \(\seq{\|Rx_k\|}[k\in K_2]\) is still ensured as long as \(\seq{\sigma_k}\notin\ell_1\).
%However, quasi-Fejér monotonicity as in \Cref{thm:General:QF} still holds even for summable \(\seq{\sigma_k}\).
%\end{rem}



==> TeX/Text/SuperMann/Comparisons.tex <==
\subsubsection{Hybrid global and local phase algorithms}
\emph{Blind} \(K_0\)-updates in \refSM[] are inspired from \cite[Alg. 1]{chen1999proximal}, and so is the notation \(K_0=\set{k_0,k_1,\ldots}\).

\emph{Educated} \(K_1\)- and \emph{safeguard} \(K_2\)-updates instead play the role of \emph{inner}- and \emph{outer-phases} in the general algorithmic framework described in \cite[§5.3]{izmailov2014newton} for finding a zero of a candidate merit function \(\varphi\) (e.g. \(\varphi(x)=\frac12\|Rx\|^2\) in our case).
Differently from \cite[Alg. 5.16]{izmailov2014newton} where all previous inner-phase iterations are discarded as soon as the required sufficient decrease is not met, the \refSM[] allows for an alternation of phases that eventually stabilizes on the fast local one, provided the solution is sufficiently regular.
Our scheme is more in the flavor of \cite[Alg. 5.19]{izmailov2014newton}, although with less conservative requirements for triggering \emph{inner} \(K_1\)-updates (\(\varphi(x^{k+1})\) is here compared with \(\varphi(x^k)\), whereas in the cited scheme with the smallest past value).
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Line-search for KM}
The recent work \cite{giselsson2016line} proposes an acceleration of the classical KM scheme for finding a fixed point of an \avg{} operator \(T\) based on a line search on the relaxation parameter.
Namely, instead of the \emph{nominal} update
\(
	\bar x=T_\lambda x
\)
with \(\lambda\in[0,\nicefrac1\alpha]\) as in \eqref{eq:KM}, values \(\lambda'>\nicefrac1\alpha\) are first tested and the update
\(
	x^+=T_{\lambda'} x
\)
is accepted as long as
\(
	\|Rx^+\|\leq\hat c\|R\bar x\|
\)
holds for some constant \(\hat c\in(0,1)\).
Convergence is significantly enhanced in practice for many applications, and the method is particularly attractive when \(T=S_2\circ S_1\) is the composition of an affine mapping \(S_1\) and a cheap operator \(S_2\), in which case the line search is computationally inexpensive.

In the setting of the \refSM[], this corresponds to selecting \(d^k=-Rx^k\), discarding \emph{blind} updates (\ie setting \(c=0\)), foretracking \emph{educated} updates and using plain KM iterations as safeguard steps.
However, though preserving the same theoretical convergence guarantees of KM (hence of the \refSM[]), it does not improve its best-case local linear rate.
Moreover, \emph{educated} updates as in \cite{giselsson2016line} compare with the \emph{nominal} KM safeguard, resulting in a possibly more conservative line search --- since \(\|R(Tx)\|\leq\|Rx\|\) (cf. \cref{lem:AvgProp:KMResDecrease}), and in a waste of KM iterations whenever nominal steps are discarded.

%For the sake of global convergence of the \refSM[], the stepsize \(\tau_k\) can be anything as long as it is upper bounded and either one of the conditions \(K_0,K_1,K_2\) is satisfied.
%However, the scheme is tailored for directions \(\seq{d^k}\) as if
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Smooth optimization with envelope functions}
For solving nonsmooth minimization problems in composite form, \cite{patrinos2013proximal,patrinos2014douglas} introduced \emph{forward-backward envelope} (FBE) and \emph{Douglas-Rachford envelope} (DRE) functions.
The original nonsmooth problem is recast into the minimization of continuous (possibly continuously differentiable) real-valued exact penalty functions closely related to forward-backward and Douglas-Rachford splittings, named \emph{envelopes} due to their kinship with the Moreau \emph{envelope} and the Proximal Point Algorithm.
This paved the way for the employment of fast methods for smooth unconstrained minimization problems \cite{patrinos2013proximal,patrinos2014douglas,stella2016forward}, or for globalizing convergence of fast methods for solving nonlinear equations \cite{themelis2016forward}.

%In \cite{giselsson2016nonsmooth} a universal envelope function is proposed that generalizes the FBE and DRE when one of the functions in the composite minimization problem is quadratic.
%Universal envelopes go beyond this, however, as they cover the wider range of problems \eqref{eq:Problem} not necessarily arising from optimization.
%Many favorable properties of such envelopes are proven, opening the possibility to apply the same techniques so far only discussed for forward-backward and Douglas-Rachford splittings in optimization to a larger variety of problems.

Though envelope functions have proven very effective, their employment is limited to composite operators as described above.
The \refSM[] instead offers a unifying framework that is based uniquely on evaluations of the nonexpansive mapping \(T\), regardless of their structure.






